Migrate when necessary: toward partitioned reclaiming for soft real-time tasks

This paper presents a new strategy for scheduling soft real-time tasks on multiple identical cores. The proposed approach is based on partitioned CPU reservations and it uses a reclaiming mechanism to reduce the number of missed deadlines. We introduce the possibility for a task to temporarily migrate to another, less charged, CPU when it has exhausted the reserved bandwidth on its allocated CPU. In addition, we propose a simple load balancing method to decrease the number of deadlines missed by the tasks. The proposed algorithm has been evaluated through simulations, showing its effectiveness (compared to other multi-core reclaiming approaches) and comparing the performance of different partitioning heuristics (Best Fit, Worst Fit and First Fit).

==> artifact.tex <==

\section{Artifact description}

The artifact contains all the executables, code source, graph
generators, as well as the shell scripts of running them. To validate
the results, run the test scripts and check the graph curve with the
paper's graphs. The source code is multiplatform, however this
artifact desctiption is only for debian linux. Please notice that all
the tools used in this work are free and open source.



You can run our simulations in two ways: with a virtual machine or
with source code.
\subsection{With virtual machine}
First, you need to download the artifact virtual machine by running
the following command:

\begin{minted}{bash}
 $ wget http://houssam.univ-lille1.fr/RTNS_ARTIFACT.ova
\end{minted}

Once, the virtual machine is downloaded, you may need to download and
install \emph{virtual box} tool. Dowload and installation instructions
can be found on this link :

\url{https://www.virtualbox.org/wiki/Linux_Downloads}


Once Virtual box is installed, you need to import the downloaded file
by clicking on \emph{file $>$ import a virtual application}.

This operation may take several minutes. When the operation ends, you
can start the virtual machine. 

After that the virtual machine has fully run its boot, you may follow
this tutorial starting from section \ref{sec:instal}. The performances
may be downgraded if you choose to run a virtual machine and
simulations may take a longer time compared to the second method.


\subsection{With source code}
First of all, the artifact can be downloaded by running the command:

\begin{minted}{bash}
 $ git clone https://github.com/zahoussem/reclaiming_simulator
\end{minted}

 
Some tools are needed to compile and run the simulations and generate
the graphs. Here is a list of these tools and how to download and
install them:


\begin{itemize}
\item \textbf{R}: is an open source programming language and software
  environment for statistical computing and graphics that is supported
  by the R Foundation for Statistical Computing. R is used to generate
  jobs execution times and also to do the statistical analysis and
  plotting them. To install R, please execute the following commands:


\begin{minted}{bash}
$ sudo add-apt-repository "https://<miroir.cran>/bin/linux/<version.ubuntu>/"
$ sudo add-apt-repository "deb https://stat.ethz.ch/CRAN/bin/linux/ubuntu zesty/"
$ sudo apt-key adv --keyserver keyserver.ubuntu.com --recv-keys E084DAB9
$ sudo apt-get update
$ sudo apt-get install r-base r-base-dev
\end{minted}

You may need to install R packages \emph{reshape}, \emph{lattice} by
running on R console the commands
\begin{minted}{bash}
$ R
$ > install.packages("Package_name") 
\end{minted}



\item \textbf{Scala:} Our tool is built with scala. Scala is a
  functionnal and object-oriented programming language.  Scala code is
  compiled to java byte code and run on java virtual machine. Hence,
  open jdk must also be installed. You may need to install the latest
  release for java which is compatible with the sbt (will be discribed
  later). To install scala, please, execute the following commands:


\begin{minted}{bash}
$ wget www.scala-lang.org/files/archive/scala-2.11.7.deb
$ sudo dpkg -i scala-2.11.7.deb
\end{minted}

If you have not java 8 installed \footnote{please notice that all
  earlier java versions must be removed, otherwise sbt will crach}, you
  may execute the following commands:
\begin{minted}{bash}
$ sudo apt-get install python-software-properties
$ sudo add-apt-repository ppa:webupd8team/java
$ sudo apt-get update
$ sudo apt-get install oracle-java8-installer
\end{minted}




\item Scala Build Tool (SBT): This tool is used to build and run scala
  project in an interactive mode. this tool can be downloaded by
  running the following commands on your console:
\end{itemize}

\begin{minted}{bash}
$ echo "deb https://dl.bintray.com/sbt/debian /" | sudo tee -a /etc/apt/sources.list.d/sbt.list
$ sudo apt-key adv --keyserver hkp://keyserver.ubuntu.com:80 --recv 2EE0EA64E40A89B84B2DF73499E82A75642AC823
$ sudo apt-get update
$ sudo apt-get install sbt
\end{minted}


\subsection{Artifact Installation \& Execution}
\label{sec:instal}
Once sbt is installed: You can compile and run the project by
executing the following commands: \footnote{[download\_path is the
  home directory of the virtual machine]}

\begin{minted}{bash}
$ cd [download_path]/reclaiming_simulator/Artifact
$ sbt compile
$ sbt run
\end{minted}


Once the execution is completed, the results file is generated in your
"tmp" folder. to generate \emph{similar} graphs as those of the
paper, you need to run the \emph{RTNSArtifact.R} R-script by executing
the command:

\begin{minted}{bash}
$ Rscript --vanilla RTNSArtifact.R 
\end{minted}

PDF file(s) will be created in the current folder. Please open it
using okular or evince to visualiz the plots.

\subsection{Artifact contents}
This artifact contains the source code in Scala, bash scripts and R
scripts. The Source code is compound of 6 packages:
\begin{enumerate}
\item \textbf{task:} Contains all task related classes.
\item \textbf{archi:} Contains all architecture related classes and a
  part of the simulation code. This Implementation is inpired from the
  linux kernel implementation.
\item \textbf{sim:} Contains the simulation engine for both global and
  partitioned schedulers
\item \textbf{generator:} Contains all scripts used to generate task
  sets and scenarios.
\item \textbf{GUI:} Contains two classes to generate automatically
  gant diagrams (typically used for small scenario)
\item \textbf{main:} Contains the main class, lunchers, and
  simulations parameters.
\end{enumerate}

\subsubsection{Datasets generation}
To modify the simulation parameters, you need to modify the class
\emph{main.Main.scala}. Several generation methods are
available. Please refer to the class \emph{generator.Generator.scala}.

==> figs/grubexample.tex <==
\begin{tikzpicture}
    
    \draw [line width = 0.5mm, ->](10,5)--(10,6);
    \node at (10.5,5.2){\Large $\mathsf{a}_{i1}$};
    
    \draw [line width = 0.5mm, <-, red!90!black](10,3.8)--(10,4.8);
    \node at (11.2,4){\Large $\mathsf{a}_{i1}+ \mathsf{T}_i$};
    
    \draw [line width = 0.5mm, <-, color=blue!70!red](13,5)--(13,6);
    \node at (13.8,5.2){\Large $1^{st} \mathsf{d}_i$ };
    
    \draw [line width = 0.5mm, <-, green!50!yellow](13,3.8)--(13,4.8);
    \node at (13.8,4){\Large $2^{nd} \mathsf{d}_i$};
    
    %% first task
    \def\d{0}
    \draw (0,0)--(22,0);
    \foreach \i in {0,1,...,22}
             {
               \draw (\i,0+\d)--(\i,-0.5+\d);
             }
             \draw [line width = 0.5mm, ->](0,0)--(0,2);
             \draw [line width = 0.5mm,  color=red](10,0)--(10,2);
             \draw [line width = 0.5mm, <-,
             color=blue!70!red](10.05,0)--(10.05,2);
             \draw [line width = 0.5mm, <-,
             color=green!50!red](20,0)--(20,2);
             
             \draw [line width = 0.5mm, <-,
color=blue!70!red](9,0-6)--(9,2-6);
             \draw [line width = 0.5mm, <-,
color=green!50!red](17,0-6)--(17,2-6);
             
             \draw [fill,color= red, opacity=0.3](0,0)rectangle(1,1);
             \draw [fill,color= red, opacity=0.3](7,0)rectangle(10,1);
             \draw [fill,color= red, opacity=0.3](11,0)rectangle(12,1);
             
             
             
             \node at (0,-1-1){0};
             \node at (1,-1-1){1};
             \node at (2,-1-1){1};
             \node at (3,-1-1){1};
             \node at (4,-1-1){1};
             \node at (5,-1-1){1};
             \node at (6,-1-1){1};
             \node at (7,-1-1){1};
             \node at (8,-1-1){4.5};
             \node at (9,-1-1){8};
             \node at (10,-1-1){11.5};
             \node at (11,-1-1){11.5};
             \node at (12,-1-1){12.5};
             \node at (13,-1-1){12.5};
             \node at (14,-1-1){12.5};
             \node at (15,-1-1){12.5};
             \node at (16,-1-1){12.5};
             \node at (17,-1-1){12.5};
             \node at (18,-1-1){12.5};
             \node at (19,-1-1){12.5};
             \node at (20,-1-1){12.5};
             \node at (21,-1-1){12.5};
             \node at (22,-1-1){12.5};
             \node at (-1,-1) {\textbf{\large $\mathsf{t}$}};
             \node at (-1,-1-1) {\textbf{\large $\mathsf{V}_1$}};
             \def\d{1}
             \node at (0,-1+\d-1){0};
             \node at (1,-1+\d-1){1};
             \node at (2,-1+\d-1){2};
             \node at (3,-1+\d-1){3};
             \node at (4,-1+\d-1){4};
             \node at (5,-1+\d-1){5};
             \node at (6,-1+\d-1){6};
             \node at (7,-1+\d-1){7};
             \node at (8,-1+\d-1){8};
             \node at (9,-1+\d-1){9};
             \node at (10,-1+\d-1){10};
             \node at (11,-1+\d-1){11};
             \node at (12,-1+\d-1){12};
             \node at (13,-1+\d-1){13};
             \node at (14,-1+\d-1){14};
             \node at (15,-1+\d-1){15};
             \node at (16,-1+\d-1){16};
             \node at (17,-1+\d-1){17};
             \node at (18,-1+\d-1){18};
             \node at (19,-1+\d-1){19};
             \node at (20,-1+\d-1){20};
             \node at (21,-1+\d-1){21};
             \node at (22,-1+\d-1){22};
             
             
             \node at (0,2.5){$\mathsf{a}_{i1}$};
             
             \node at (0.5,1.5){Ex};
             \node at (1.5,1.5){Ry};
             \node at (2.5,1.5){Ry};
             \node at (3.5,1.5){Ry};
             \node at (4.5,1.5){Ry};
             \node at (5.5,1.5){Ry};
             \node at (6.5,1.5){Ry};
             \node at (7.5,1.5){Ex};
             \node at (8.5,1.5){Ex};
             \node at (9.5,1.5){Ex};
             \node at (10.5,1.5){Ry};
             \node at (11.5,1.5){Rx};
             \node at (12.5,1.5){Wt};
             \node at (13.5,1.5){Ed};
             \node at (14.5,1.5){Ed};
             \node at (15.5,1.5){Ed};
             \node at (16.5,1.5){Ed};
             \node at (17.5,1.5){Ed};
             \node at (18.5,1.5){Ed};
             \node at (19.5,1.5){Ed};
             
             
             
             
             
             
             


% \draw [fill,color= red, opacity=0.3](11,0)rectangle(12,1);


%\draw (0,0)--(15,-1);

%% second task 
\def\d{-6}
\draw (0,0+\d)--(22,0+\d);
\foreach \i in {0,1,...,22}
{
\draw (\i,0+\d)--(\i,-0.5+\d);
}
\draw [line width = 0.5mm, ->](1,0+\d)--(1,2+\d);
\draw [fill,color= green, opacity=0.3](1,0+\d)rectangle(7,1+\d);
\draw [fill,color= green, opacity=0.3](10,0+\d)rectangle(11,1+\d);
\draw [line width = 0.5mm, <-, color=red](11,0+\d)--(11,2+\d);
\def\d{-5}
\node at (0,-1+\d-1){0};
\node at (1,-1+\d-1){1};
\node at (2,-1+\d-1){2};
\node at (3,-1+\d-1){3};
\node at (4,-1+\d-1){4};
\node at (5,-1+\d-1){5};
\node at (6,-1+\d-1){6};
\node at (7,-1+\d-1){7};
\node at (8,-1+\d-1){8};
\node at (9,-1+\d-1){9};
\node at (10,-1+\d-1){10};
\node at (11,-1+\d-1){11};
\node at (12,-1+\d-1){12};
\node at (13,-1+\d-1){13};
\node at (14,-1+\d-1){14};
\node at (15,-1+\d-1){15};
\node at (16,-1+\d-1){16};
\node at (17,-1+\d-1){17};
\node at (18,-1+\d-1){18};
\node at (19,-1+\d-1){19};
\node at (20,-1+\d-1){20};
\node at (21,-1+\d-1){21};
\node at (22,-1+\d-1){22};
\def\d{-6}


\node at (1,-1+\d-1){1};
\node at (2,-1+\d-1){2.4};
\node at (3,-1+\d-1){3.8};
\node at (4,-1+\d-1){5.2};
\node at (5,-1+\d-1){6.6};
\node at (6,-1+\d-1){8};
\node at (7,-1+\d-1){9.4};
\node at (8,-1+\d-1){9.4};
\node at (9,-1+\d-1){9.4};
\node at (10,-1+\d-1){9.4};
\node at (11,-1+\d-1){10.8};
\node at (12,-1+\d-1){10.8};
\node at (13,-1+\d-1){10.8};
\node at (14,-1+\d-1){10.8};
\node at (15,-1+\d-1){10.8};
\node at (16,-1+\d-1){10.8};
\node at (17,-1+\d-1){10.8};
\node at (18,-1+\d-1){10.8};
\node at (19,-1+\d-1){10.8};
\node at (20,-1+\d-1){10.8};
\node at (21,-1+\d-1){10.8};
\node at (22,-1+\d-1){10.8};


\node at (1.5,1.5+\d){Ex};
\node at (2.5,1.5+\d){Ex};
\node at (3.5,1.5+\d){Ex};
\node at (4.5,1.5+\d){Ex};
\node at (5.5,1.5+\d){Ex};
\node at (6.5,1.5+\d){Ex};
\node at (7.5,1.5+\d){Ry};
\node at (8.5,1.5+\d){Ry};
\node at (9.5,1.5+\d){Ry};
\node at (10.5,1.5+\d){Ex};
\node at (11.5,1.5+\d){Ed};
\node at (12.5,1.5+\d){Ed};
\node at (13.5,1.5+\d){Ed};
\node at (14.5,1.5+\d){Ed};
\node at (15.5,1.5+\d){Ed};
\node at (16.5,1.5+\d){Ed};
\node at (17.5,1.5+\d){Ed};
\node at (18.5,1.5+\d){Ed};
\node at (19.5,1.5+\d){Ed};




\node at (-1,-1+\d+1) {\textbf{\large $\mathsf{t}$}};
\node at (-1,-1-1+\d) {\textbf{\large $\mathsf{V}_1$}};
\end{tikzpicture}

